Mother of Dragons: A Massive, quiescent core in the dragon cloud (IRDC G028.37+00.07)

Context: Core accretion models of massive star formation require the existence of massive, starless cores within molecular clouds. Yet, only a small number of candidates for such truly massive, monolithic cores are currently known. Aims: Here we analyse a massive core in the well-studied infrared-dark cloud (IRDC) called the 'dragon cloud' (also known as G028.37+00.07 or 'Cloud C'). This core (C2c1) sits at the end of a chain of a roughly equally spaced actively star-forming cores near the centre of the IRDC. Methods: We present new high-angular resolution 1 mm ALMA dust continuum and molecular line observations of the massive core. Results: The high-angular resolution observations show that this region fragments into two cores C2c1a and C2c1b, which retain significant background-subtracted masses of 23 Msun and 2 Msun (31 Msun and 6 Msun without background subtraction), respectively. The cores do not appear to fragment further on the scales of our highest angular resolution images (0.200 arcsec, 0.005 pc ~ 1000 AU). We find that these cores are very dense (nH2 > 10^6 cm-3) and have only trans-sonic non-thermal motions (Ms ~ 1). Together the mass, density and internal motions imply a virial parameter of < 1, which suggests the cores are gravitationally unstable, unless supported by strong magnetic fields with strengths of ~ 1 - 10 mG. From CO line observations, we find that there is tentative evidence for a weak molecular outflow towards the lower-mass core, and yet the more massive core remains devoid of any star formation indicators. Conclusions: We present evidence for the existence of a massive, pre-stellar core, which has implications for theories of massive star formation. This source warrants follow-up higher-angular-resolution observations to further assess its monolithic and pre-stellar nature.

==> AUTHORS.tex <==
%%%% PLEASE ADD YOU DETAIL BELOW 


%%% E.G. 

A.T.Barnes
Argelander-Institut f\"{u}r Astronomie, Universit\"{a}t Bonn, Auf dem H\"{u}gel 71, 53121, Bonn, Germany

J. Liu
East Asian Observatory, 660 N. A‘ohok¯u Place, University Park, Hilo, HI, USA

Q. Zhang
Center for Astrophysics | Harvard \& Smithsonian, Cambridge, MA, USA

%%% Append below.... 
Jonathan C. Tan
Chalmers University \& Univ. of Virginia

Ke Wang
Kavli Institute for Astronomy and Astrophysics, Peking University, 5 Yiheyuan Road, Haidian District, Beijing 100871, China

Jaime E. Pineda
Max-Planck-Institut f\"ur extraterrestrische Physik, Giessenbachstrasse 1, D-85748 Garching, Germany

Wanggi Lim
IPAC, Mail Code 100-22, Caltech, 1200 E. California Boulevard, Pasadena, CA 91125, USA

Richard J. Parker\thanks{Royal Society Dorothy Hodgkin Fellow}
Department of Physics and Astronomy, The University of Sheffield, Hicks Building, Hounsfield Road, Sheffield, S3 7RH, UK

\author[0000-0001-9656-7682]{Jonathan~D.~Henshaw}
\affiliation{Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK}
\affiliation{Max-Planck-Institut f\"ur Astronomie, K\"onigstuhl 17, D-69117 Heidelberg, Germany}

David-Sebastian Kalb (D.-S. Kalb)
Max Plank Institute for Astronomy (MPIA), Königstuhl 17, D-69117 Heidelberg, Germany

\author[0000-0002-3078-9482]{\'Alvaro S\'anchez-Monge}
\affiliation{Observatorio Astron\'omico Nacional (OAN, IGN), Calle Alfonso XII 3, 28014, Madrid, Spain}




A.~T.~Barnes, 
J.~Liu, 
Q.~Zhang
J.~C.~Tan
P.~Caselli
G.~Cosentino
F.~Fontani 
J.~D.~Henshaw
I.~Jiménez-Serra
D-S.~Kalb 
C.~Y.~Law
S.~N.~Longmore 
R.~J.~Parker
J.~E.~Pineda
A.~S\'anchez-Monge
W.~Lim
K.~Wang

==> Paper -- Astronomy and Astrophysics -- Cloud C cores -- arxiv/AUTHORS.tex <==
%%%% PLEASE ADD YOU DETAIL BELOW 


%%% E.G. 

A.T.Barnes
Argelander-Institut f\"{u}r Astronomie, Universit\"{a}t Bonn, Auf dem H\"{u}gel 71, 53121, Bonn, Germany

J. Liu
East Asian Observatory, 660 N. A‘ohok¯u Place, University Park, Hilo, HI, USA

Q. Zhang
Center for Astrophysics | Harvard \& Smithsonian, Cambridge, MA, USA

%%% Append below.... 
Jonathan C. Tan
Chalmers University \& Univ. of Virginia

Ke Wang
Kavli Institute for Astronomy and Astrophysics, Peking University, 5 Yiheyuan Road, Haidian District, Beijing 100871, China

Jaime E. Pineda
Max-Planck-Institut f\"ur extraterrestrische Physik, Giessenbachstrasse 1, D-85748 Garching, Germany

Wanggi Lim
IPAC, Mail Code 100-22, Caltech, 1200 E. California Boulevard, Pasadena, CA 91125, USA

Richard J. Parker\thanks{Royal Society Dorothy Hodgkin Fellow}
Department of Physics and Astronomy, The University of Sheffield, Hicks Building, Hounsfield Road, Sheffield, S3 7RH, UK

\author[0000-0001-9656-7682]{Jonathan~D.~Henshaw}
\affiliation{Astrophysics Research Institute, Liverpool John Moores University, 146 Brownlow Hill, Liverpool L3 5RF, UK}
\affiliation{Max-Planck-Institut f\"ur Astronomie, K\"onigstuhl 17, D-69117 Heidelberg, Germany}

David-Sebastian Kalb (D.-S. Kalb)
Max Plank Institute for Astronomy (MPIA), Königstuhl 17, D-69117 Heidelberg, Germany

\author[0000-0002-3078-9482]{\'Alvaro S\'anchez-Monge}
\affiliation{Observatorio Astron\'omico Nacional (OAN, IGN), Calle Alfonso XII 3, 28014, Madrid, Spain}




A.~T.~Barnes, 
J.~Liu, 
Q.~Zhang
J.~C.~Tan
P.~Caselli
G.~Cosentino
F.~Fontani 
J.~D.~Henshaw
I.~Jiménez-Serra
D-S.~Kalb 
C.~Y.~Law
S.~N.~Longmore 
R.~J.~Parker
J.~E.~Pineda
A.~S\'anchez-Monge
W.~Lim
K.~Wang
